Simplicity Bias in Transformers and their Ability to Learn Sparse Boolean Functions

Despite the widespread success of Transformers on NLP tasks, recent works have found that they struggle to model several formal languages when compared to recurrent models. This raises the question of why Transformers perform well in practice and whether they have any properties that enable them to generalize better than recurrent models. In this work, we conduct an extensive empirical study on Boolean functions to demonstrate the following: (i) Random Transformers are relatively more biased towards functions of low sensitivity. (ii) When trained on Boolean functions, both Transformers and LSTMs prioritize learning functions of low sensitivity, with Transformers ultimately converging to functions of lower sensitivity. (iii) On sparse Boolean functions which have low sensitivity, we find that Transformers generalize near perfectly even in the presence of noisy labels whereas LSTMs overfit and achieve poor generalization accuracy. Overall, our results provide strong quantifiable evidence that suggests differences in the inductive biases of Transformers and recurrent models which may help explain Transformer's effective generalization performance despite relatively limited expressiveness.

==> sections/limitations.tex <==
\section{Limitations}\label{sec:Limitations}

A general limitation of this line of work is that most of the results are primarily confined to artificial datasets. Although such formal languages provide us with a controlled setting and clarity regarding the precise nature of the problem, the relation to practical tasks remains unclear. Hence, while our results highlight the contrast in the performance between the two types of architectures, its precise implications on real-world tasks remain unclear.


There are two negative results that do not support our hypothesis. (a) All the experiments discussed in the main paper are on strings of fixed lengths. We conducted some experiments on tasks with variable length sequences which in some sense have low sensitivity. The tasks can be seen as a variable length extension of sparse parities and sparse majorities. Unlike the fixed length setting, we found both LSTMs and Transformers perform similarly on those tasks. See Section \ref{app:varlen} in the Appendix for more details. (b) Although we found Transformers to consistently converge to low sensitivity functions in the case of Boolean functions, we did not find similar behaviour on sentiment classification datasets such as SST and IMDB.

A caveat with empirical studies such as this is that the results depend on the hyperparameters and other aspects of the experimental setup. While we have tried to be as thorough as possible with hyperparameter tuning, there is always a chance that the results or behaviour could differ for some hyperparameter.



